Multi-Scale Dense Networks for Resource Efficient Image Classification

In this paper we investigate image classification with computational resource limits at test time. Two such settings are: 1. anytime classification, where the network's prediction for a test example is progressively updated, facilitating the output of a prediction at any time; and 2. budgeted batch classification, where a fixed amount of computation is available to classify a set of examples that can be spent unevenly across "easier" and "harder" inputs. In contrast to most prior work, such as the popular Viola and Jones algorithm, our approach is based on convolutional neural networks. We train multiple classifiers with varying resource demands, which we adaptively apply during test time. To maximally re-use computation between the classifiers, we incorporate them as early-exits into a single deep convolutional neural network and inter-connect them with dense connectivity. To facilitate high quality classification early on, we use a two-dimensional multi-scale network architecture that maintains coarse and fine level features all-throughout the network. Experiments on three image-classification tasks demonstrate that our framework substantially improves the existing state-of-the-art in both settings.

==> Cost_Sensitive_CNN - arXiv-20180607/ablation.tex <==
%!TEX root=main.tex

\subsection{Ablation study}
\label{sec:ablation}


We perform additional experiments to shed light on the contributions of the three main components of \methodnameshort{}, \emph{viz.}, multi-scale feature maps, dense connectivity, and intermediate classifiers.

 \begin{wrapfigure}{r}{0.48\textwidth}
      \centering
            \vspace{-1 ex}
      \includegraphics[width=0.48\textwidth]{figures/MSDNet_var.pdf}
      \vspace{-2 ex}
      \caption{Ablation study (on CIFAR-100) of \methodnameshort{}s  that shows the effect of dense connectivity, multi-scale features, and intermediate classifiers. Higher is better.
     }\vspace{-2ex}
      \label{fig:ablation}
\end{wrapfigure}

We start from an \methodnameshort{} with six intermediate classifiers and remove the three main components one at a time. To make our comparisons fair, we keep the computational costs of the full networks similar, at around $3.0\times 10^{8}$ FLOPs, by adapting the network width, i.e., number of output channels at each layer. After removing all the three components in an \methodnameshort{}, we obtain a regular VGG-like convolutional network. We show the classification accuracy of all classifiers in a model in the left panel of \figurename~\ref{fig:ablation}. Several observations can be made: 1. the dense connectivity is crucial for the performance of \methodnameshort{} and removing it hurts the overall accuracy drastically (orange vs. black  curve); 2. removing multi-scale convolution hurts the accuracy only in the lower budget regions, which is consistent with our motivation that the multi-scale design introduces discriminative features early on; 3. the final canonical CNN (star) performs similarly as MSDNet under the specific budget that matches its evaluation cost exactly, but it is unsuited for varying budget constraints. The final CNN performs substantially better at its particular budget region than the model without dense connectivity (orange curve). This suggests that dense connectivity is particularly important in combination with multiple classifiers.

%while it is not suitable for budgeted learning. Although we can train multiple independent CNNs of varying sizes, they can not reuse features of each other, and lead to inferior performances as shown earlier.

%
%For fair comparison, we attach six intermediate classifiers to all networks (except the one without intermediate classifier), and let them have roughly $3.0\times 10^{8}$ FLOPs by adapting the network width, i.e., number of output channels at each layer. We show the classification accuracy of all classifiers in a model in \figurename~\ref{fig:ablation}, from which several observations can be made: (1) removing any of the three parts causes a significant accuracy loss to MSDNets; (2) without multi-scale convolution, the network is able to yield acceptable results at the last classifier, while the performance of early classifiers are underwhelming; (3) removing dense connections hurt the overall accuracy drastically, although the performance gap between an early classifier and the final classifier is relatively smaller.
%


==> Cost_Sensitive_CNN - arXiv-20180607/abstract.tex <==
%!TEX root=main.tex
In this paper we investigate image classification with computational resource limits at test time. Two such settings are: 1. \emph{anytime classification}, where the network's prediction for a test example is progressively updated, facilitating the output of a prediction at any time; and 2. \emph{budgeted batch classification}, where a fixed amount of computation is available to classify a set of examples that can be spent unevenly across ``easier'' and ``harder'' inputs. 
In contrast to most prior work, such as the popular Viola and Jones algorithm, our approach is based on convolutional neural networks. We train multiple classifiers with varying resource demands, which we adaptively apply during test time. 
To maximally re-use  computation between the classifiers, we incorporate them as early-exits into a single deep convolutional neural network and inter-connect them with dense connectivity. To facilitate high quality classification early on, we use a two-dimensional multi-scale network architecture that maintains coarse and fine level features all-throughout the network. 
%Such an approach would typically lead to a significant reduction in accuracy due to the interference of classifiers with learned features---and it would lead to inaccurate intermediate classification results due to the lack of course-scale features early on in the network. 
%To avoid interference between classifiers and feature creation we  dense connectivity and introduces shared multi-scale representations to obtain coarse level features all-throughout the network. To our knowledge, this is the first principled solution to these two challenges that arise with intermediate classifiers in neural networks. 
%We develop a new network architecture that performs on par with state-of-the-art convolutional networks, whilst facilitating prediction in two  settings:
Experiments on three image-classification tasks demonstrate that our framework substantially improves the existing state-of-the-art in both settings.
%resource efficient classification.
%the efficacy of our architecture, in particular, when measured in terms of classification accuracy as a function of the amount of compute available.

%This paper studies convolutional networks that require limited computational resources at test time. We develop a new network architecture that performs on par with state-of-the-art convolutional networks, whilst facilitating prediction in two  settings: (1) an \emph{anytime-prediction} setting in which the network's prediction for one example is progressively updated, facilitating the output of a prediction at any time; and (2) a \emph{batch computational budget} setting in which a fixed amount of computation is available to classify a set of examples that can be spent unevenly across ``easier'' and ``harder'' examples. Our network architecture uses multi-scale convolutions and progressively growing feature representations, which allows for the training of multiple classifiers at intermediate layers of the network. Experiments on three image-classification datasets demonstrate the efficacy of our architecture, in particular, when measured in terms of classification accuracy as a function of the amount of compute available.

%This paper addresses the problem of doing inference with deep convolutional neural networks (CNNs) under limited computational resource. We consider the following two scenarios: 1) the \emph{anytime} setting where there is a nondeterministic time budget $B$, which is a random variable following a known distribution. At test time, a prediction is needed to be retrieved whenever a stochastic time budget is met. This requires the model to produce accurate predictions quickly, but still be able to keep improving the performance when budget allows. 2) there is no fixed time budget, but we would like to minimize the overall evaluation time by reducing the cost on predicting easy examples. For these purposes, we propose a novel CNN architecture which incorporates the idea from Neural Fabrics \cite{saxena2016convolutional} of performing down-sampling early in the network to ensure high accuracy under small time budget, and the idea from DenseNets \cite{huang2016densely} of introducing the dense connectivity to encourage feature reusing in an efficient way. The resulting network can be trained end-to-end conveniently to maximize the expected accuracy over the budget distribution. It is also able to early exit easy examples to save expected evaluation time. We show on multiple datasets that the network can be trained efficiently and is able to produce significantly more accurate predictions over the budget distribution.



==> Cost_Sensitive_CNN - arXiv-20180607/anytimeresults.tex <==
%!TEX root=./main.tex





% \begin{figure}[t]
%%\vspace{-2 ex}
%      \centering
%      \includegraphics[width=0.4\textwidth]{figures/anytime-imagenet.pdf}\\
%            \vspace{-2 ex}
%      \caption{Anytime classification performance of \methodnameshort{} and ensemble of ResNets with varying depths on ImageNet.}
%      \label{fig:anytime-imagenet}
%      \vspace{-2 ex}
%\end{figure}



\vspace{-1ex}
\subsection{Anytime Prediction}
\label{sec:anytime}
In the anytime prediction setting, the model maintains a progressively updated distribution over classes, and it can be forced to output its most up-to-date prediction at an arbitrary time.

\textbf{Baselines.}
There exist several baseline approaches for anytime prediction: FractalNets \citep{fractalnet}, deeply supervised networks \citep{dsn}, and ensembles of deep networks of \emph{varying} or \emph{identical} sizes.
FractalNets allow for multiple evaluation paths during inference time, which vary in computation time. In the anytime setting, paths are evaluated in order of increasing computation. In our result figures, we replicate the FractalNet results reported in the original paper \citep{fractalnet} for reference.
Deeply supervised networks introduce multiple early-exit classifiers throughout a network, which are applied on the features of the particular layer they are attached to. Instead of using the original model proposed in \cite{dsn}, we use the more competitive ResNet and DenseNet architectures (referred to as \emph{DenseNet-BC} in \cite{huang2016densely}) as the base networks in our experiments with deeply supervised networks. We refer to these as
\emph{ResNet$^\text{MC}$} and \emph{DenseNet$^\text{MC}$}, where $MC$ stands for \emph{multiple classifiers}. Both networks require about $1.3\times 10^8$ FLOPs when fully evaluated; the detailed network configurations are presented in the supplementary material.
%
In addition, we include ensembles of ResNets and DenseNets of \emph{varying} or \emph{identical} sizes. At test time, the networks are evaluated sequentially (in ascending order of network size) to obtain predictions for the test data. All predictions are averaged over the evaluated classifiers.
%
%and a more competitive, and \emph{unpublished}, variant of DenseNets (denoted as \emph{DenseNet*}), that is optimized to maximize FLOP efficiency by doubling the growth rate after each transition layer.
On ImageNet, we compare \methodnameshort{} against a highly competitive ensemble of ResNets  and DenseNets, with depth varying from 10 layers to 50 layers, and 36 layers to 121 layers, respectively.
%The depths for ResN varying from 10 layers to 50 layers. All the models are the same as those described in \cite{resnet}, except the ResNet-10 and ResNet-26, which are variants of ResNet-18 that were modified by removing/adding one residual block from/to each of the last four spatial resolutions in the network.


%are the same five architectures we used in the experiments with the batch computational budget setting (that is, ResNets with 10, 18, 26, 34, and 50 layers, respectively). We order these networks by network size in ascending order, and evaluate them sequentially at test time.

%We always start with the network with minimum cost, and keep evaluating larger and larger models if budget allows. The predictions from the evaluated networks can be ensembled to further boost the performance. We implement this idea using the state-of-the-art ResNets \citep{resnet} and DenseNets (with bottleneck structure and dimension reduction at transition layer) \citep{huang2016densely}. Note that the initial design of DenseNet was more parameter efficiency oriented, it is not competitive in terms computational efficiency. Although we adopt the dense connectivity in our model, we follow the ResNets to produce doubled feature maps at a coarser scale. To make comparisons fair, we apply the same strategy to DenseNet, yielding a far more competitive baseline.


%first consider a uniform distribution on $[0, 5\times 10^{8}]$ (FLOPs) for the budget. The upper bound of the distribution is chosen in accordance with the widely used 110-layer ResNet \citep{resnet} on CIFAR datasets, which has about $5\times 10^8$ FLOPs. As mentioned in early sections, the exponential distribution is very common for test time budget in the real world. We consider an exponential distribution with the same mean as the uniform distribution. We also consider two artificial distributions: 1) linear grow distribution, whose probability density function (p.d.f.) linearly grows on $[0, 5\times 10^{8}]$; 2) tower shape distribution, whose p.d.f. peaks at $2.5\times 10^8$, and linearly decay to 0 at $0$ and $5\times 10^{8}$.

%\textbf{Details of architecture.}
%The \methodnameshort{} used in our anytime-prediction experiments has 24 layers (each layer corresponds to a column in Fig.~\ref{fig:layout}), using the reduced network with transition layers as described in Section \ref{sec:network}. The classifiers operate on the output of the $2\!\times\!(i\!+\!1)^{\text{th}}$ layers, with $i\!=\!1,\ldots,11$. On ImageNet, we use an \methodnameshort{} with 23 multi-scale layers, and the $i^\text{th}$ classifier operates on the $(4i\!+\!3)^{\text{th}}$ layer (with $i\!=\!1,\ldots,5$). For simplicity, the losses of all the classifiers are weighted equally during training.

%On ImageNet, we use the same \methodnameshort{} as describe in previous subsection. The loss associated with each classifier is either weighted equally, or it is weighted using the budget distribution $p(B)$ if that distribution is known.

 \begin{figure*}[t]
      \centering
\vspace{-2 ex}
%      \includegraphics[width=0.32\textwidth]{figures/anytime-cifar10-final1.pdf}
\centerline{\includegraphics[width=0.48\textwidth]{figures/anytime-imagenet.pdf}
      \includegraphics[width=0.48\textwidth]{figures/anytime-cifar100-final1.pdf}}
    \vspace{-1 ex}
      \caption{Accuracy (\emph{top-1}) of \emph{anytime prediction} models as a function of computational budget on the ImageNet (left) and CIFAR-100 (right) datasets. Higher is better.}
       \vspace{-2 ex}
     \label{fig:anytime}
\end{figure*}
\textbf{Anytime prediction results}  are presented in Figure~\ref{fig:anytime}. The left plot shows the top-1 classification accuracy on the ImageNet validation set.
%The left panel shows the  results on ImageNet of \methodnameshort{} and ResNet ensemble.
Here, for all budgets in our evaluation, the accuracy of \methodnameshort{} substantially outperforms the ResNets and DenseNets ensemble. In particular, when the budget ranges from $0.1\!\times\! 10^{10}$ to $0.3\!\times \!10^{10}$ FLOPs, \methodnameshort{} achieves $\sim \! 4\%\!-\!8\%$ higher accuracy.
%The strong performance of \methodnameshort{} on ImageNet shows that reusing feature representations in challenging tasks can be even more beneficial.




We evaluate more baselines on CIFAR-100 (and CIFAR-10; see supplementary materials). We observe that \methodnameshort{} substantially outperforms ResNets$^\text{MC}$ and DenseNets$^\text{MC}$ at any computational budget within our range. This is due to the fact that after just a few layers, \methodnameshort{}s have produced low-resolution feature maps that are much more suitable for classification than the high-resolution feature maps in the early layers of ResNets or DenseNets. \methodnameshort{} also outperforms the other baselines for nearly all computational budgets, although it performs on par with ensembles when the budget is very small. In the extremely low-budget regime, ensembles have an advantage because their predictions are performed by the first (small) network, which is optimized exclusively for the low budget.
However, the accuracy of ensembles does not increase nearly as fast when the budget is increased. The \methodnameshort{} outperforms the ensemble as soon as the latter needs to evaluate a second model: unlike \methodnameshort{}s, this forces the ensemble to repeat the computation of similar low-level features repeatedly. Ensemble accuracies saturate rapidly when all networks are shallow.


%\begin{wrapfigure}{r}{0.45\textwidth}
%       \vspace{-4 ex}
%       \includegraphics[width=0.45\textwidth]{figures/anytime-cifar10-dis-final1.pdf}
%      \caption{Classification accuracies of our anytime prediction models on the CIFAR-10 dataset using three different budget distributions $P(B)$.}
%       \vspace{-2 ex}
%     \label{fig:anytime-cifar10-dis}
%\end{wrapfigure}
%
%\paragraph{Budget Distribution}
%To investigate to what extent the performance of \methodnameshort{}s in the Anytime setting depends on the budget distribution $P(B)$, we perform experiments with three different budget distributions. The three distributions are illustrated in Figure~\ref{fig:anytime-cifar10-dis} as dotted lines: a uniform distribution, an exponential distribution and a normal distribution. During training we assign weights $w_k$ proportional to the probability that the forced exit will result in an exit after classifier $f_k$. The results in Figure~\ref{fig:anytime-cifar10-dis} show that the accuracy distributions are somewhat shifted based on the weight assignments, however, no drastic changes occur. This result provides some reassurance that the uniform weighting is probably a good choice in many real-world applications, and that we do not need to worry too much about errors in our estimates of $p(B)$.





%The saturation  may be reduced by including increasingly deep models (labeled as \emph{varying depth}), which has the downside that (unlike \methodnameshort{}s) computations of similar low-level features are repeated multiple times.

%As a result, the ensembles

%The margin of improvement over ensemble methods widens with the budget, as ensembles increasingly waste computation as they do not re-use extract features across ensemble members. On the flip-side,

%Here, the ensemble approaches have an advantage over \methodnameshort{}s, because we evaluate the smallest models in our ensembles first. In contrast to the first classifier(s) in our model, the features learned by these models are completely optimized to give rise immediate classifications, whereas the feature representations learned by \methodnameshort{} also need to maintain more complex features that are relevant for predictions produced by later classifiers. As a result, the ``effective capacity'' of our initial classifier (at the same number of FLOPs) is lower than that of the smallest models in the ensembles. However, this pays off quickly with increasing test time budget.





%Taken together, the results in the figure demonstrate the strong potential of \methodnameshort{}s. For budget distributions $P(B)$ in which low budget assignments are likely, we surmise that an ensemble of a very small DenseNet and a \methodnameshort{} may be able to achieve even slightly better results (for reasons explained in the previous paragraph). We did not experiment with such hybrid approaches in this study, because the optimal hybrid approach would strongly depend on the choice for $P(B)$.




% $0$ and $3 \! \times \! 10^{8}$ FLOPs\footnote{The maximum FLOPs value coincides with the FLOPs needed for making a prediction using a ResNet-62.}. We experiment with

%\subsection{Image Segmentation}
%\textbf{Dataset}
%We perform image segmentation on Camvid dataset, which contains 367, 101, and 233 images in size $360 \! \times \! 480$ for training, validation, and testing respectively. Each image is of the size The task is to predict the class of each pixel in an image. There are 12 classes, but the pixels in the \textit{void} class are omitted during evluation.
%
%\textbf{Training details.}
%We simply follow same training prosedures in the image experiment setting except for the following differences: 1) All segmentation models are trained for 200 epochs, and the learning rate is divided by a factor of 10 every 50 epochs. 2) The weight decay is $2 \! \times \! 10^{-4}$. 3) The training images weren't randomly cropped, but we still randomly flip the images horizontally.
%
%\subsubsection{Anytime Prediction}
%
%
%
%\textbf{Baseline.}
%The state-of-the-art framework for image segmentation, Fully Convolutional DenseNet (FC-DenseNet) \citep{jegou2016one}, is considered extremely parameter efficient compared to all other previous methods; therefore, it is our first choice as a baseline. We fix the depth of the FC-DenseNet to having 1, 3, 5, 7, 9, 11, 9, 7, 5, 3, and 1 layer in its 11 dense blocks respectively, and change the growth rate to meet the budget. In our early experiments, we found that given limitted computation budget,
%this architecture outperforms the one with eleven 2-layer dense blocks.
%
%\textbf{Deails of architecture.}
%To reduce the computation on large scales, we have an down-sampling block which directly connects to the input layer. It contains three $3 \!\times \! 3$  layers, one with stride $1$ and two with stride 2, which down-sample the image into one fourth of the original size.
%We feed the down-sampled features to a MSDNet with 4 scales and 6 layers.
%In image segmentation scenario, since the local information is quite important, the classifiers use the top 3 coarsest scales for prediction rather than only the coarsest scale.
%Moreover, we consider a variant of MSDNet which preserves the upsampling connections like convolutional neural fabric.
%
%\textbf{Budget distribution.}
%In this experimention, we consider the budget as a uniform distribution between $0$ and $4 \! \times \! 10^{10}$ FLOPs.
%
%
%\textbf{Results.}




==> Cost_Sensitive_CNN - arXiv-20180607/archdetails.tex <==
%!TEX root=./main.tex


\section{Details of MSDNet Architecture and Baseline Networks}
\label{sec:archdetails}
We use \methodnameshort{} with three scales on the CIFAR datasets, and the network reduction method introduced in \ref{subsec:arch} is applied. \autoref{fig:reduction} gives an illustration of the reduced network.
The convolutional layer functions in the first layer, $h_{1}^s$, denote a sequence of $3 \! \times \! 3$ convolutions (Conv), batch normalization (BN;~\cite{batch-norm}), and rectified linear unit (ReLU) activation. In the computation of $\tilde h_{1}^s$, down-sampling is performed by applying convolutions using strides that are powers of two. For subsequent feature layers, the transformations $h_{\ell}^s$ and $\tilde h_{\ell}^s$ are defined following the design in DenseNets \citep{huang2016densely}: Conv($1\times 1$)-BN-ReLU-Conv($3\times 3$)-BN-ReLU. We set the number of output channels of the three scales to 6, 12, and 24, respectively. Each classifier has two down-sampling convolutional layers with 128 dimensional $3 \! \times \! 3$ filters, followed by a $2 \! \times \! 2$ average pooling layer and a linear layer.

The \methodnameshort{} used for ImageNet has four scales, respectively producing 16, 32, 64, and 64 feature maps at each layer. The network reduction is also applied to reduce computational cost. The original images are first transformed by a 7$\times$7 convolution and a 3$\times$3 max pooling (both with stride 2), before entering the first layer of \methodnameshort{}s. The classifiers have the same structure as those used for the CIFAR datasets, except that the number of output channels of each convolutional layer is set to be equal to the number of its input channels.

\renewcommand{\arraystretch}{1.1}
\begin{figure}[!h]
%\vspace{1 ex}
\centerline{
\includegraphics[width=0.8\textwidth]{figures/reduction.pdf}}
\caption{Illustration of an MSDNet with network reduction. The network has $S\!=\!3$ scales, and it is divided into three blocks, which maintain a decreasing number of scales. A transition layer is placed between two contiguous blocks. }
\label{fig:reduction}
\vspace{-3 ex}
\end{figure}




\textbf{Network architecture for anytime prediction.}
The \methodnameshort{} used in our anytime-prediction experiments has 24 layers (each layer corresponds to a column in Fig. 1 of the main paper), using the reduced network with transition layers as described in Section 4. The classifiers operate on the output of the $2\!\times\!(i\!+\!1)^{\text{th}}$ layers, with $i\!=\!1,\ldots,11$. On ImageNet, we use \methodnameshort{}s with four scales, and the $i^\text{th}$ classifier operates on the $(k\!\times\! i\!+\!3)^{\text{th}}$ layer (with $i\!=\!1,\ldots,5$ ), where $k\!=\!4,6$ and $7$. For simplicity, the losses of all the classifiers are weighted equally during training.


\textbf{Network architecture for budgeted batch setting.} The \methodnameshort{}s used here for the two CIFAR datasets have depths ranging from 10 to 36 layers, using the reduced network with transition layers as described in Section~4. The $k^{\text{th}}$ classifier is attached to the $(\sum_{i=1}^k i) {}^{\text{th}}$ layer. The  \methodnameshort{}s used for ImageNet are the same as those described for the anytime learning setting.

\textbf{ResNet$^\text{MC}$ and DenseNet$^\text{MC}$.}
The \emph{ResNet$^\text{MC}$} has 62 layers, with $10$ residual blocks at each spatial resolution (for three resolutions): we train early-exit classifiers on the output of the 4$^{\text{th}}$ and 8$^{\text{th}}$ residual blocks at each resolution, producing a total of $6$ intermediate classifiers (plus the final classification layer). The \emph{DenseNet$^\text{MC}$} consists of 52 layers with three dense blocks and each of them has 16 layers. The six intermediate classifiers are attached to the 6$^{\text{th}}$ and 12$^{\text{th}}$ layer in each block, also with dense connections to all previous layers in that block.



==> Cost_Sensitive_CNN - arXiv-20180607/batchresults.tex <==
%!TEX root=./main.tex

\vspace{-1.5 ex}
\subsection{Budgeted batch classification}
\vspace{-1 ex}
\label{sec:batch-budget}
In budgeted batch classification setting, the predictive model receives a batch of $M$ instances and a computational budget $B$ for classifying all $M$ instances. In this setting, we use \emph{dynamic evaluation}: we perform \emph{early-exiting} of ``easy'' examples at early classifiers whilst propagating ``hard'' examples through the entire network, using the procedure described in Section~\ref{sec:network}.

%Specifically, we associate each classifier with a confidence threshold, and let a test example exit from the first classifier at which it obtains sufficiently confident prediction, \emph{i.e.}, its maximum soft-max value is no less than the threshold at that classifier. The confidence threshold $\theta_k$ at the $k^{\text{th}}$ classifier is determined using the validation set, such that a proportion of $q_{k}\!=\! z (1-q)^{k-1}q$ validation samples exit from this classifier (where $z$ is a normalizing constant). In our preliminary experiments, we also try associating each class with an independent threshold, but it gives no significant improvement.


\textbf{Baselines.} On ImageNet, we compare the dynamically evaluated \methodnameshort{} with five ResNets \citep{resnet} and five DenseNets \citep{huang2016densely}, AlexNet \citep{alexnet}, and GoogleLeNet \citep{szegedy2015going}; see the supplementary material for details.
%We do not compare with the popular VGG network \citep{simonyan2014very} as it is far less competitive in terms of efficiency compared to ResNet: a 16-layer VGG model achieves a similar accuracy as ResNet-26, while has 5 times more FLOPs.
We also evaluate an ensemble of the five ResNets that uses exactly the same dynamic-evaluation procedure as \methodnameshort{}s at test time: ``easy'' images are only propagated through the smallest ResNet-10, whereas ``hard'' images are classified by all five ResNet models (predictions are averaged across all evaluated networks in the ensemble). We classify batches of $M \! = \! 128$ images.

On CIFAR-100, we compare \methodnameshort{} with several highly competitive baselines, including ResNets~\citep{resnet},  DenseNets~\citep{huang2016densely} of varying sizes, Stochastic Depth Networks \citep{stochastic}, Wide ResNets \citep{wide} and FractalNets \citep{fractalnet}. We also compare \methodnameshort{} to the ResNet$^\text{MC}$ and DenseNet$^\text{MC}$ models that were used in Section~\ref{sec:anytime}, using dynamic evaluation at test time. We denote these baselines as \emph{ResNet$^\text{MC}$ / DenseNet$^\text{MC}$ with early-exits}. To prevent the result plots from becoming too cluttered, we present CIFAR-100 results with dynamically evaluated ensembles in the supplementary material. We classify batches of $M \! = \! 256$ images at test time.

%We do not experiment with deeper models as they are unlikely to be more competitive.

%Our final baseline is obtained by applying the dynamic evaluation strategy to an ensemble of independently trained networks with increasing depth (we use the most competitive DenseNet* architecture). If a test input obtains an insufficiently confident prediction at a shallower network, it will be further evaluated by a deeper one, until its prediction is confident enough or it reaches the deepest model. We assign the confidence thresholds as described for \methodnameshort{}. It is worth noting that for each test input this baseline re-uses computation by ensembling the predictions of all evaluated networks. We refer to this baseline as \emph{Dynamic Ensemble of DenseNets*}.




%All the models used here are the same as those described in the original papers, except that the ResNet-10 and ResNet-26 are variants of ResNet-18 that were modified by removing/adding one residual block from/to each of the last four spatial resolutions in the network.




\textbf{Budgeted batch classification results} on ImageNet are shown in the left panel of Figure~\ref{fig:early-exit}. We trained three \methodnameshort{}s with different depths, each of which covers a different range of computational budgets. We plot the performance of each \methodnameshort{} as a gray curve; we select the best model for each budget based on its accuracy on the validation set, and plot the corresponding accuracy as a black curve.
The plot shows that the predictions of \methodnameshort{}s with dynamic evaluation are substantially more accurate than those of ResNets and DenseNets that use the same amount of computation. For instance, with an average budget of $1.7 \! \times \! 10^{9}$ FLOPs, \methodnameshort{} achieves a top-1 accuracy of $\sim$75\%, which is $\sim$6\% higher than that achieved by a ResNet with the same number of FLOPs. Compared to the computationally efficient DenseNets, \methodnameshort{} uses $\sim \!2\! -\! 3\times$ times fewer FLOPs to achieve the same classification accuracy. Moreover, \methodnameshort{} with dynamic evaluation allows for very precise tuning of the computational budget that is consumed, which is not possible with individual ResNet or DenseNet models. The ensemble of ResNets or DenseNets with dynamic evaluation performs on par with or worse than their individual counterparts (but they do allow for setting the computational budget very precisely).

The right panel of Figure~\ref{fig:early-exit} shows our results on CIFAR-100.  The results show that \methodnameshort{}s consistently outperform all baselines across all budgets. Notably, \methodnameshort{} performs on par with a 110-layer ResNet using only 1/10th of the computational budget and it is up to $\sim \! 5$ times more efficient than DenseNets, Stochastic Depth Networks, Wide ResNets, and FractalNets.
%, whilst achieving higher accuracies than all these networks when there are no computational constraints.
Similar to results in the anytime-prediction setting, \methodnameshort{} substantially outperform ResNets$^{MC}$ and DenseNets$^{MC}$ with multiple intermediate classifiers, which provides further evidence that the coarse features in the MSDNet are important for high performance in earlier layers.

%is consistent with our believe that earlier features in convolution networks are ill suited for immediate classification.




%The results of \methodnameshort{} on ImageNet shown in the right panel of Figure~\ref{fig:early-exit} is also promising.

% \begin{figure}[t]
%%\vspace{-2 ex}
%      \centering
%      \includegraphics[width=0.48\textwidth]{figures/imagenet-visual.pdf}\\
%            %\includegraphics[width=0.5\textwidth]{figures/visual_earlyexit_cifar10-2.pdf}
%      \vspace{-2 ex}
%      \caption{Random example images from the ImageNet classes \emph{Red wine} and \emph{Volcano}. Top row: images exited from the first classification layer of a \methodnameshort{} with correct prediction; Bottom row: images failed to be correctly classified at the first classifier but were correctly predicted and exited at the last layer.}
%      \label{fig:early-exit-visualize_cifar10}
%     \vspace{-3 ex}
%\end{figure}





 \begin{wrapfigure}{r}{0.48\textwidth}
      \centering
      \vspace{-2 ex}
      \includegraphics[width=0.48\textwidth]{figures/imagenet-visual.pdf}\\
            %\includegraphics[width=0.5\textwidth]{figures/visual_earlyexit_cifar10-2.pdf}
      \vspace{-1 ex}
      \caption{Sampled images from the ImageNet classes \emph{Red wine} and \emph{Volcano}. Top row: images exited from the first classifier of a \methodnameshort{} with correct prediction; Bottom row: images failed to be correctly classified at the first classifier but were correctly predicted and exited at the last layer.}
      \vspace{-2 ex}
      \label{fig:early-exit-visualize_cifar10}
\end{wrapfigure}
\textbf{Visualization.}
To illustrate the ability of our approach to reduce the computational requirements for classifying ``easy'' examples, we show twelve randomly sampled test images from two ImageNet classes in Figure~\ref{fig:early-exit-visualize_cifar10}. The top row shows ``easy'' examples that were correctly classified and exited by the first classifier. The bottom row shows ``hard'' examples that would have been incorrectly classified by the first classifier but were passed on because its uncertainty was too high. The figure suggests that early classifiers recognize prototypical class examples, whereas the last classifier recognizes non-typical images.


 \begin{figure*}[t]
\vspace{-2 ex}
%     \includegraphics[width=0.32\textwidth]{figures/early-exit-cifar10.pdf}
\centerline{
      \includegraphics[width=0.48\textwidth]{figures/early-exit-imagenet-2.pdf}
\includegraphics[width=0.48\textwidth]{figures/early-exit-cifar100.pdf}
      }
          \caption{Accuracy (top-1) of \emph{budgeted batch classification} models as a function of average computational budget per image the on ImageNet (left) and CIFAR-100 (right) datasets. Higher is better.}
               \vspace{-2 ex}
      \label{fig:early-exit}
\end{figure*}







%, as defined in eq.~(\ref{eq:ql}).
%Here, $z$ is a normalization factor to ensure that $q_{k}$'s sum to one.

%compensate for the fact that we truncate layers with exit probability less than $\epsilon$ (we set $\epsilon=0.03$ in our experiment) at training.

%\danlu{add one paragraph}

%\textbf{Early-exit with a confidence threshold.} In our model, we implement an dynamic evaluation (called early-exit) by evaluating the classifiers sequentially in our \methodnameshort{} on the instances in the validation set. We record the soft-max predictions of the samples arrived at a classification layer (all the samples are evaluated at the first classifier), and sort them in descending order according the maximum soft-max probability. Next, we define a threshold for each classifier between that determines whether or not that classifier can make a decision on an image: if the maximum value in the classifier's predictive distribution is higher than the threshold, that classifier makes the decision and outputs the highest-scoring class, but the prediction is deferred to the next classifier when it is smaller than the threshold.

%Moreover, we assume the probability of a test sample exits successfully from the $k^{\text{th}}$ classifier follows the geometric distribution $r(Y = k) = (1-p)^{k-1}p$.
%The value of $p$ can be solved by letting the expected evaluation cost meet our given budget $B$.
%Then we use the validation set to find a threshold $t_k$ such that a fraction of $r(k)$ samples exit from the $k^{\text{th}}$ classifier. Practically, the layers with exit probability smaller than a small number $\epsilon$ \footnote{we set $\epsilon=0.03$ in our experiment} are removed to save both training and testing time.
%[To do: option 1]
%We estimate the threshold for each classifier in such a way as to ensure that at least $p$\% of the decisions that that classifier makes on the validation set is correct. Each possible value of $p$ corresponds to a budget value $B$: we estimate the relation between $p$ and $B$ on the validation set, too, and use it to decide on an appropriate threshold value for a given budget $B$.

%We assume a test sample exits from the $k^{th}$ classifier with probability $(1-p)p^{k-1}$. The value of $p$ can be solved by letting the expected evaluation cost meet our given budget $B$. Then we use the validation set to find the threshold such that a fraction of $r(k)=(1-p)p^{k-1}$ samples exit from the $k^{th}$ classifier. Practically, the layers with exit probability smaller than a small number $\epsilon$ (we set $\epsilon=0.03$ in our experiment) are removed to save both training and testing time.

%\danlu{rewrite the following paragraph}

%\textbf{Details of architecture.} The \methodnameshort{}s used here for the two CIFAR datasets have depths ranging from 10 to 36 layers, using the reduced network with transition layers as described in Section~\ref{sec:network}. The $k^{\text{th}}$ classifier is attached to the $(\sum_{i=1}^k i) {}^{\text{th}}$ layer.
%The network used for ImageNet is the same as that described in the previous subsection.

%We assign the classifier weights $w_\ell$ as described in Section~\ref{sec:method} and set the \methodnameshort{} depth by truncating all layers with less than $\epsilon\!=\!3\%$ examples exiting.

% \begin{wrapfigure}{r}{0.45\textwidth}
%      \centering
%            \vspace{-2 ex}
%      \includegraphics[width=0.45\textwidth]{figures/ablation-v3.pdf}\\
%            %\includegraphics[width=0.5\textwidth]{figures/visual_earlyexit_cifar10-2.pdf}
%      \vspace{-1 ex}
%      \caption{Remove dense connections, multi-scale convolutions or intermediate classifiers from a MSDNet.}
%      \vspace{-2 ex}
%      \label{fig:ablation}
%\end{wrapfigure}



%The DenseNets* outperform most of the other baselines, but they do not achieve the same performance as \methodnameshort{}s. Moreover, using first type of baselines in computational-budget settings requires us to keep many models in memory; this is a substantial limitation, in particular, when the budget varies a lot. By contrast, \methodnameshort{}s have the property that we can tune the threshold to increase or decrease the expected evaluation cost. To be able to change the budget $B$ at inference time, we only need to maintain a set of thresholds, as opposed to a set of models.

%Given the relatively strong performance of DenseNets*, we apply our early-exit strategy to an ensemble of such networks with increasing depth, by treating each network as a classifier in \methodnameshort{}. Therefore, if a test example obtains insufficiently confident prediction at a shallower network, it will be further evaluated by a deeper one, until its prediction is confident enough or it reaches the deepest model.



%The dynamically evaluated DenseNets* ensemble (shown by the solid green curve in Figure~\ref{fig:early-exit}) performs quite competitively on CIFAR-10, suggesting that our early-exit strategy can be potentially applied to an ensemble of convolutional networks of varying sizes. On CIFAR-100 and ImageNet, however, the ensemble only performs on par with its single-model counterpart, potentially because of a lack of consistency in the predictions of the independently trained models. In contrast, \methodnameshort{} benefits from the joint training process, leading it to consistently outperform all the baselines on both datasets.



% \begin{figure}[t]
%%\vspace{-2 ex}
%      \centering
%      \includegraphics[width=0.4\textwidth]{figures/early-exit-imagenet.pdf}\\
%            \vspace{-2 ex}
%      \caption{Top-1 accuracy as a function of average computational cost budget (per image) on ImageNet.}
%      \label{fig:early-exit-imagenet}
%      \vspace{-2 ex}
%\end{figure}



==> Cost_Sensitive_CNN - arXiv-20180607/conclusion.tex <==
%!TEX root=main.tex
 \vspace{-2 ex}
 \section{Conclusion}
 \vspace{-1ex}
We presented the \methodnameshort{}, a novel convolutional network architecture, optimized to incorporate CPU budgets at test-time. Our design is based on two high-level design principles, to generate and maintain coarse level features throughout the network and to inter-connect the layers with dense connectivity. The former allows us to introduce intermediate classifiers even at early layers and the latter ensures that these classifiers do not interfere with each other. The final design is a two dimensional array of horizontal and vertical layers, which decouples depth and feature coarseness. Whereas in traditional  convolutional networks features only become coarser with increasing depth, the {MSDNet} generates features of all resolutions from the first layer on and maintains them throughout. The result is an architecture with an unprecedented range of efficiency. A single network can outperform all competitive baselines on an impressive range of computational budgets ranging from highly limited CPU constraints to almost unconstrained settings.

As future work we plan to investigate the use of resource-aware deep architectures beyond object classification, \emph{e.g.} image segmentation~\citep{fcn}. Further, we intend to explore approaches that combine \methodnameshort{}s with model compression~\citep{chen2015compressing,HanMD15}, spatially adaptive computation \citep{figurnov2016spatially} and more efficient convolution operations \citep{chollet2016xception,howard2017mobilenets} to further improve computational efficiency.

%hybrid approaches, for instance, by constructing an ensemble of a few very small classification models and our architecture. The models may be combined in an approaches that average predictions as well as in cascaded approaches.



==> Cost_Sensitive_CNN - arXiv-20180607/intro.tex <==
%!TEX root = main.tex
\section{Introduction}

% talking points:
% - horses
% - one network for several mobile devices 
% - 24,000 ( https://qz.com/472767/there-are-now-more-than-24000-different-android-devices/ )

%
Recent years have witnessed a surge in demand for applications of visual object recognition, for instance, in self-driving cars~\citep{bojarski2016end} and content-based image search \citep{wan2014deep}.
This demand has in part been fueled through the promise generated by the  astonishing progress of convolutional networks (CNNs) on visual object recognition benchmark
%~\citep{alexnet,vgg,szegedy2015going,huang2016densely,fcn}. This development was in part driven by several public
competition datasets, such as ILSVRC \citep{deng2009imagenet} and COCO \citep{lin2014microsoft}, where state-of-the-art models may have even surpassed human-level performance~\citep{he2015delving,resnet}.

\begin{wrapfigure}{r}{0.3\textwidth}
\vspace{-2ex}
      \includegraphics[width=0.3\textwidth]{figures/horsefaces.pdf}
      \vspace{-3ex}
      \caption{Two images containing a \emph{horse}. The left image is canonical and easy to detect even with a small model, whereas the right image requires a computationally more expensive network architecture. (Copyright Pixel Addict and Doyle (CC BY-ND 2.0).)}
      \label{fig:horseface}
\vspace{-2.5ex}
\end{wrapfigure}However, the requirements of such competitions differ from real-world applications, which tend to incentivize  resource-hungry models with high computational demands at inference time. For example, the COCO 2016 competition was won by a large ensemble of computationally intensive CNNs\footnote{\url{http://image-net.org/challenges/talks/2016/GRMI-COCO-slidedeck.pdf}} --- a model likely far too computationally expensive for any resource-aware application. 
%To obtain high accuracy, such large models are necessary because they need to capture rare images. 
Although much smaller models would also obtain decent error, very large, computationally intensive models seem necessary to correctly classify the hard examples that make up the bulk of the remaining misclassifications of modern algorithms.  To illustrate this point, Figure~\ref{fig:horseface} shows two images of horses. The left image depicts a horse in canonical pose and is easy to classify, whereas the right image is taken from a rare viewpoint and is likely in the tail of the data distribution. Computationally intensive models are needed to classify such tail examples correctly, but are wasteful when applied to canonical images such as the left one. 

In real-world applications, computation directly translates into power consumption, which should be minimized for environmental and economical reasons, and is a scarce commodity on mobile devices. This begs the question: \emph{why do we choose between either wasting computational resources by applying an unnecessarily computationally expensive model to easy images, or making mistakes by using an efficient model that fails to recognize difficult images?} Ideally, our systems should automatically use small networks when test images are easy or computational resources limited, and use big networks when test images are hard or computation is abundant. 


%For most of the common test-cases a small energy efficient model would suffice. However, occasional samples require drastically more expensive models to be classified correctly. 

% After all, super-human accuracy in pedestrian detection is of little use if the prediction is delivered after the car has already hit the person.

Such systems would be beneficial in at least two settings with computational constraints at test-time: \emph{anytime prediction}, where the network can be forced to output a prediction at any given point in time; and \emph{budgeted batch classification}, where a fixed computational budget is shared across a large set of examples which can be spent unevenly across ``easy'' and ``hard'' examples.
%
A practical use-case of anytime prediction is in mobile apps on Android devices: in 2015, there existed $24,093$ distinct Android devices\footnote{Source: \url{https://opensignal.com/reports/2015/08/android-fragmentation/}}, each with its own distinct computational limitations. It is infeasible to train a different network that processes video frame-by-frame at a fixed framerate for each of these devices. Instead, you would like to train a single network that maximizes accuracy on all these devices, within the computational constraints of that device. 
%The anytime setting is applicable to, for example, self-driving cars, which need to process high-resolution video streams on-the-fly and may need to output a prediction immediately when an unexpected event occurs. 
%The budgeted batch classification setting is a common scenario in web services that process large number of images with fixed resources \citep{deepspeech2}. For example, as of 2010, Google Image Search had over 10 Billion images indexed\footnote{\url{https://en.wikipedia.org/wiki/Google_Images}}, which has likely grown to over 1 Trillion since. Even if a new model to process these images is only 1/10s slower per image, it would add 3170 years of CPU time. Here, systems may increase their average accuracy by reducing the amount of computation spent on ``easy'' cases and applying the saved computation on ``difficult'' cases. 
The budget batch classification  setting is ubiquitous in large-scale machine learning applications. Search engines, social media companies, on-line advertising agencies,  all must process large volumes of data on limited hardware resources.  For example, as of 2010, Google Image Search had over 10 Billion images indexed\footnote{\url{https://en.wikipedia.org/wiki/Google_Images}}, which has likely grown to over 1 Trillion since. Even if a new model to process these images is only 1/10s slower per image, this additional cost would add 3170 years of CPU time. 
In the budget batch classification setting, companies can improve the  average accuracy by reducing the amount of computation spent on ``easy'' cases to save up computation for ``hard'' cases. 
%Companies routinely have to trade-off  the cost of larger models with their benefits. 

%Computer vision has a long and successful history of CPU-budget aware detection and classification. Most prominently the work by~\cite{viola2001robust,viola2001rapid} (with over 30,000 combined citations) has famously enabled real-time face detection on mobile devices or safe-search features in search engines. 
%%Although these settings have only recently become increasingly the focus of academic research~\citep{ICML2012Xu_592,zhu2017sequential,trapeznikov2013supervised,nan2017adaptive}, we would like to argue that they constitute the dominant settings in industrial applications. To be profitable corporations need to be cost-effective, and their products, such as image classification, must be strictly within (computational) budget. 
%%Digital cameras use the resource adaptive algorithm by ~\cite{viola2001robust} to find faces in images in real-time and Safe-Search features in search engines~\citep{fleck1996finding} can only afford the classification of Billions of images because pictures that are easily identified as benign can be quickly sorted out with minimum computational effort. 
%This work and the majority of its follow-up work~\citep{xu2013cost,ICML2012Xu_592,xu2014classifier} is based on boosted trees.
%Boosted trees learn ensembles of classifiers that greedily reduce the remaining residual one tree at a time and are a natural fit for resource limited classification. If the resource limits during test-time are unknown, one can boost for a large number of trees and stop the evaluation once the CPU time is depleted or the classification sufficiently certain (through early exits). Because of the greedy ordering this procedure obtains the same results as if the models had been trained explicitly for these specific budgets. 

%the evaluation is topped after a small subset of the trees and the prediction is identical to that of a classifier trained for that exact computational budget 

%Even in the most na\"ive setting, if two classifiers are trained on the same data set under different tree budgets, $b_1$ and $b_2$ respectively (with $b_1<b_2$), then the first $b_1$ trees of both classifiers are identical. It is therefore only natural to stop the execution of a classifier if sufficient certainty is reached or the resource budget exceeded, as it was effectively classified by the exact classifier trained for that budget. 

%In the wake of CNNs it is natural to ask how to enable similar accuracy/cost trade-offs with deep learning. Analogous to the trees %in boosting, CNNs process the input one layer at a time. However, in this paper we argue that in contrast to boosting,

Motivated by prior work in computer vision on resource-efficient recognition \citep{viola2001robust}, we aim to develop CNNs that ``slice'' the computation and process these slices one-by-one, stopping the evaluation once the CPU time is depleted or the classification sufficiently certain (through ``early exits''). Unfortunately, the architecture of CNNs is inherently at odds with the introduction of early exits. CNNs learn the data representation and the classifier jointly, which leads to two problems with early exits: 1. The features in the last layer are extracted directly to be used by the classifier, whereas earlier features are not. The inherent dilemma is that different kinds of features need to be extracted depending on how many layers are left until the classification. 2. The features in different layers of the network may have different scale. Typically, the first layers of a deep nets operate on a fine scale (to extract low-level features), whereas later layers transition (through pooling or strided convolution) to coarse scales that allow global context to enter the classifier. Both scales are needed but happen at different places in the network. 

% Perhaps the most na\"ive approach is to independently/jointly train multiple networks of increasing capacity, and sequentially evaluate them at test time~\citep{zhu2017sequential}. However, a clear downside of this approach is that the representation can not be reused across networks, even for the highly sharable low-level features.  As CNNs are computationally expensive (much more than e.g. decision trees), this computation should not go wasted. 

%We therefore propose a convolutional network architecture with an internal cascade of intermediate classifiers, which is able to produce accurate predictions quickly, and still can keep improving the performance when budget allows. These intermediate classifiers 

We propose a novel network architecture that addresses both of these problems through careful design changes, allowing for resource-efficient image classification. Our network uses a cascade of intermediate classifiers throughout the network. The first problem, of classifiers altering the internal representation, is addressed through the introduction of dense connectivity \citep{huang2016densely}. By connecting all layers to all classifiers, features are no longer dominated by the most imminent early-exit and the trade-off between early or later classification can be performed elegantly as part of the loss function. 
The second problem, the lack of coarse-scale features in early layers, is addressed by adopting a multi-scale network structure. At each layer we produce features of all scales (fine-to-coarse), which facilitates good classification early on but also extracts low-level features that only become useful after several more layers of processing. Our network architecture is illustrated in Figure~\ref{fig:layout}, and we refer to it as \emph{\methodnamecap{} (\methodnameshort{})}.


%We find that na\"ively attaching internal classifiers to state-of-the-art deep networks, e.g., Residual Networks (ResNets) \citep{resnet}, yields poor performance. These intermediate classifiers not only have low accuracy themselves, but also degrades the final classifier (see \autoref{fig:ablation}, more discussions are given in Section~\ref{sec:network}). 


%(Figure~\ref{fig:layout}), which we refer to as \emph{\methodnamecap{} (\methodnameshort{})}. Despite their limited depth,
%the intermediate classifiers are competitive because of two crucial components of \methodnameshort{}s:  \emph{multi-scale feature maps} and \emph{dense connectivity} \citep{huang2016densely}. The multi-scale feature maps produce high-level feature representations that are amenable to classification early on.  The dense connectivity pattern allows the network to reuse and bypass existing features  from prior layers  and ensures high accuracies in later layers.



%a search engine receives a large number of queries per second and may increase its average accuracy by reducing the amount of computation spent on simple queries and spending the saved computation on more complex queries.

%These two components are crucial for us to introduce accurate early-exit classifiers throughout the network, as shown by our experiments. We refer to our architecture as .

 \begin{figure*}[t]
      \centering
      \vspace{-4 ex}
      \includegraphics[width=\textwidth]{figures/neuralfabrics_new.pdf}
      \vspace{-0 ex}
      \caption{Illustration of the first four layers of an \methodnameshort{} with three scales. The horizontal direction corresponds to the layer direction (depth) of the network. The vertical direction corresponds to the scale of the feature maps.
Horizontal arrows indicate a regular convolution operation, whereas diagonal and vertical arrows indicate a strided convolution operation. Classifiers only operate on feature maps at the coarsest scale. Connections across more than one layer are not drawn explicitly: they are implicit through recursive concatenations.
}
      \vspace{-2 ex}
      \label{fig:layout}
\end{figure*}

%that is tailored to achieve high accuracies under computational test-time constraints. Our architecture
%Typically, deep convolutional networks learn increasingly high-level features classifiers applied to feature maps produced from early layers (on ResNets~\citep{resnet} or DenseNets~\citep{huang2016densely}) would not yield competitive results, as these are too high resolution and do not capture high-level features.


%Our experimental evaluation on three image-classification datasets demonstrates the efficacy of \methodnameshorts{}.
We evaluate \methodnameshorts{} on three image-classification datasets.
In the anytime classification setting, we show that it is possible to
provide the ability to output a prediction at any time while
maintain high accuracies throughout. In the budget batch classification setting we show that \methodnameshorts{} can be effectively used to adapt the amount of computation to the difficulty of the example to be classified, which allows us to reduce the computational requirements of our models drastically whilst performing on par with state-of-the-art CNNs in terms of overall classification accuracy. 
To our knowledge this is the first deep learning architecture of its kind that allows dynamic resource adaptation with a single model and obtains competitive results throughout. 


%In recent years, we have witnessed great advances in deep convolutional neural networks \citep{alexnet,vgg,szegedy2015going,resnet,huang2016densely,fcn}. Each year there are innovations making CNNs even more powerful, pushing the limit of prediction accuracy on challenging tasks such as the ILSVRC \citep{deng2009imagenet} and COCO competitions. On certain computer vision tasks, deep CNNs have already surpassed human-level performance \citep{he2015delving,resnet}. Meanwhile, there is a growing interests in the industry in deploying deep networks. For example, the recent success of self-driving car and content-based image search is largely attributed to powerful CNNs.

%Although unprecedented large models (or even ensembles of them) continued to set new world record scores on benchmark datasets, they are unaffordable on many real applications due to limited computational power. It is very common that in real applications people have to trade accuracy for computational time.

%In this paper, we consider two scenarios where the trade off between inference time and accuracy needs to be carefully considered. The first one is the \emph{anytime} setting where the model need to generate accurate predictions rapidly, while it should also be capable of refining the results when there is available computational budget. One example under this scenario is the vision system in a self-driving car needs to process high resolution live video streams on the fly, and respond quickly to the changing environment. The system may need to retrieve a prediction at anytime to deal with unexpected issues. The time budget to process the input is stochastic, and follows some known distributions. The second scenario is \emph{amortized cost} reduction setting, where there is no fixed budget, but we want to reduce the overall evaluation cost on the test set. The underlying assumption here is that there exists easier test samples which can be predicted with less computational cost. For example, the face detection software on a mobile phone may receive inputs with easily recognizable faces with clear background which are much easier to capture. Only those difficult images need to propagate through all the layers to get the final prediction. For another example, increasing the depth of residual networks \citep{resnet} from 101 layers to 152 layers only brings the top 1 classification error (10-crop) on the ImageNet validation set down from 21.75\% to 21.43\%. This implies that only a small portion of images need those extra layers to get the correct prediction. It could save a lot of energy if the majority of test inputs do not need to be propagated through all the layers in a deep CNN.

%Superficially, CNN has a hierarchical structure which is naturally suitable for anytime prediction or early exiting easy examples, because one can always use features from earlier layers to make predictions when necessary. However, it turns out that this naive idea does not work well, as shown in our experiment section. A main reason is that the down-sampling operations (pooling or convolution with stride larger than 1), which reduces feature maps size in CNNs, is very critical for learning high level concepts. Features without propagate through such down-sampling layers are not discriminative enough to give satisfactory predictions.

%In this paper, we introduce a novel CNN architecture to meet the requirement of the aforementioned scenarios. The proposed network is inspired by the Convolutional Neural Fabrics (CNFs) \citep{saxena2016convolutional} and DenseNets \citep{huang2016densely}. First, similar to CNFs, it introduces down-sampling operations early in the network to ensure accurate predictions without propagating test samples through many layers. Second, motivated by DenseNets, we enable later layers to reuse features learned by previous layers through dense connections. The dense connectivity also reduces the risk that later layers are affect the some aggressive features learned by early layers. Another notable advantage of the proposed method is that the network can be trained with ease in an end-to-end fashion. We show on multiple datasets it is able to give superior performances over competitive baseline algorithms.



==> Cost_Sensitive_CNN - arXiv-20180607/macros.tex <==
% METHOD NAME
\newcommand{\methodname}{multi-scale dense network}
\newcommand{\methodnamecap}{Multi-Scale DenseNet}
\newcommand{\methodblock}{dense block}
\newcommand{\methodblockcap}{Dense Block}
\newcommand{\methodnameshort}{MSDNet}
\newcommand{\methodnameshorts}{MSDNets}

\newcommand{\filler}[1]{#1}


\newcommand{\stepsizename}{growth rate}

\newcommand{\conv}[1]{$\left[\begin{array}{ll} \text{1}\times \text{1} \text{ conv}\\ \text{3}\times \text{3} \text{ conv} \end{array}\right] \times \text{#1}$}

\newcommand{\cross}[1]{#1 $\times$ #1}

% Gradients Equations
\newcommand{\feati}{x_i}
%\newcommand{\concatfeati}{x_i}
\newcommand{\clsfeati}{y_i}
\newcommand{\featk}{x_k}
\newcommand{\clsfeatk}{y_k}
\newcommand{\loss}{L}
\newcommand{\featL}{x_L}
\newcommand{\clsfeat}{y}
% Inputs and outputs
\newcommand{\anyxs}{\ensuremath{\mathbf{x}}}
\newcommand{\anyys}{\ensuremath{\mathbf{y}}}

\newcommand{\bx}{\ensuremath{\mathbf{x}}}

\newcommand{\sourcexs}{\ensuremath{\mathbf{x^\mathcal{S}}}}
\newcommand{\sourceys}{\ensuremath{\mathbf{y^\mathcal{S}}}}

\newcommand{\targetxs}{\ensuremath{\mathbf{x^\mathcal{T}}}}
\newcommand{\targetys}{\ensuremath{\mathbf{y^\mathcal{T}}}}
\newcommand{\pseudotargetys}{\ensuremath{\mathbf{\hat{y}^\mathcal{T}}}}



==> Cost_Sensitive_CNN - arXiv-20180607/method.tex <==
%!TEX root=main.tex
%\section{Cost sensitive CNN}



% \begin{wrapfigure}{r}{0.5\textwidth}
%      \centering
%      \vspace{-2 ex}
%      \includegraphics[width=0.5\textwidth]{figures/layout.pdf}
%      \vspace{-3 ex}
%      \caption{Illustration of the first five layers of an \methodnameshort{} with three scales. The horizontal direction corresponds to the layer direction (depth) of the network. The vertical direction corresponds to the scale of the feature maps.
%Horizontal arrows indicate a regular convolution operation, whereas diagonal (vertical) arrows indicate a strided convolution operation. Classifiers only operate on feature maps at the coarsest scale. Connections across more than one layer are not drawn explicitly: these connections are implicit through recursive concatenations.
%}
%      \vspace{-2 ex}
%      \label{fig:layout}
%\end{wrapfigure}




\vspace{-1ex}
\section{Problem Setup}
\vspace{-1ex}
\label{sec:setup}
We consider two settings that impose computational constraints at prediction time.


\textbf{Anytime prediction.}
In the anytime prediction setting \citep{grubb2012speedboost}, there is a finite computational budget $B \! > \! 0$ available for each test example $\bx$. The computational budget is nondeterministic, and varies per test instance. It is determined by the occurrence of an event that requires the model to output a prediction immediately.
We assume that the budget is drawn from some joint distribution $P(\bx,B)$.
In some applications $P(B)$ may be independent of $P(\bx)$ and can be estimated.
%\vspace{-2ex}
%Since it is unknown in advance if and when this event will occur, we can model the budget $B$ by a distribution $P(B)$.
%In many applications it can be estimated.
For example, if the event is governed by a Poisson process, $P(B)$ is an exponential distribution. We denote the loss of a model $f(\bx)$ that has to produce a prediction for instance $\bx$ within budget $B$ by $L(f(\bx), B)$. The goal of an anytime learner is to minimize the expected loss under the budget distribution: $L(f) = \mathbb{E}\left[ L(f(\bx), B) \right]_{P(\bx,B)}$.
%\begin{equation}
%%\vspace{-1ex}
%L(f) = \mathbb{E}\left[ L(f(\bx), B) \right]_{P(\bx,B)},
%\label{eqn:objective}
%%\vspace{-1ex}
%\end{equation}
Here, $L(\cdot)$ denotes a suitable loss function. As is common in the empirical risk minimization framework, the expectation under $P(\bx,B)$ may be estimated by an average over samples from $P(\bx,B)$.

%The anytime setting is common in scenarios where time sensitive decisions need to be made, for example, pedestrian detection in self-driving vehicles.  Here, accuracy is traded off for lower processing time. As long as the network is well-calibrated~\citep{guo2017calibration} its uncertainty estimates still allow for timely decision making. For example, in the case of pedestrian detection it is important to react fast and to err on the side of safety. The setting is also common in scenarios where a single network architecture has to process input data, such as video,  at a specific rate on   varying hardware platforms (e.g. the multitude of android phones). Here, lower accuracy is accepted to enable the application even on low-performance hardware.

%in the setting of self-driving vehicles super-human accuracy in pedestrian detection is of little use if the prediction is delivered after the car has already hit the person.

%\vspace{-2ex}
\textbf{Budgeted batch classification.}
In the budgeted batch classification setting, the model needs to classify a set of examples $\mathcal{D}_{test} \! = \! \{\bx_1,  \dots, \bx_M\}$ within a finite computational budget $B \! > \! 0$ that is known in advance. The learner aims to minimize the loss across all examples in $\mathcal{D}_{test}$ within a cumulative cost bounded by $B$, which we denote by $L(f(\mathcal{D}_{test}), B)$ for some suitable loss function $L(\cdot)$. It can potentially do so by spending less than $\frac{B}{M}$ computation on classifying an ``easy'' example whilst using more than $\frac{B}{M}$ computation on classifying a ``difficult'' example. Therefore, the budget $B$ considered here is a \emph{soft constraint} when we have a large batch of testing samples.

%The budget batch classification  setting is ubiquitous in large-scale machine learning applications. Search engines, social media companies, on-line advertising agencies,  all must process large volumes of data on limited hardware resources.  For example, as of 2010, Google Image Search had over 10 Billion images indexed\footnote{\url{https://en.wikipedia.org/wiki/Google_Images}}, which has likely grown to over 1 Trillion since. Even if a new model to process these images is only 1/10s slower per image, it would add 3170 years of CPU time. Companies routinely have to trade-off  the cost of larger models with their benefits. In the absence of specialized algorithms  they are forced to either waste computation on easy examples or increase error on difficult cases. Budgeted batch classification  addresses this trade-off explicitly.


%Practically, a cost sensitive model can only give predictions at some discrete time slot $\{\tau_1,\ldots, \tau_T\}$. Thus the test error is a constant at the time interval $[\tau_i,\tau_{i+1})$ for any $0\le \!i\! \le T$ (define $\tau_0 = 0$ and $\tau_{T+1} = +\infty$). It follows that eq. (\ref{eqn:objective}) can be simplified to
%\begin{equation}
%E = \sum_i q_i e_i,
%\label{eqn:objective-discrete}
%\end{equation}
%where $q_i=\int_{\tau_i\le B < \tau_{i+1}}P(B)$, and $e_i = \int_{\bx} {e(\bx,\tau_i)}$ is the expected test error when we retrieve predictions at time slot $\tau_i$.

%Under this setting, we assume there exist \emph{easier} test examples which require less computational cost to get their correct predictions. Cascade structured models with multiple outputs were proposed for this purpose. At test time, an input sample greedily find the cheapest exits which gives a confidence about its predictions above a given threshold. Let $\tau_i$ be the evaluation time of exiting from the $T^\text{th}$ output, we aim to minimize the overall cost $C = \sum_n \tau_{I(n)}$ on evaluating the test set while keep the accuracy less affected, where $I(n)$ the index of the output the $n^\text{th}$ test sample exits.


%\begin{figure}[t]
%\vspace{-2 ex}
%      \centering
%      \includegraphics[width=0.5\textwidth]{figures/layout.pdf}
%      \vspace{-3 ex}
%      \caption{Illustration of the first five layers of an \methodnameshort{} with three scales. The horizontal direction corresponds to the layer direction (depth) of the network. The vertical direction corresponds to the scale of the feature maps.
%Horizontal arrows indicate a regular convolution operation, whereas diagonal (vertical) arrows indicate a strided convolution operation. Classifiers only operate on feature maps at the coarsest scale.}
%      \label{fig:layout}
%\end{figure}


%\begin{wrapfigure}{r}{0.58\textwidth}
%      \centering
%\vspace{-8ex}
%      \includegraphics[width=0.28\textwidth]{figures/res-dense-intermediate.pdf}
%      \includegraphics[width=0.28\textwidth]{figures/msdnet-intermediate.pdf}
%      %\vspace{-3 ex}
%      \caption{ResNets, DenseNets (\emph{left}) and MSDNets (\emph{right}) with one intermediate classifier attached to six different internal layers (evenly spaced) ranging from shallow to deep. Dotted lines correspond to the networks without intermediate classifier.}
% \vspace{-1ex}
%     \label{fig:early-exit-demo}
%\end{wrapfigure}





 \begin{figure}[!t]
      \centering
            \vspace{-2 ex}
      \includegraphics[width=0.48 \textwidth]{figures/ablation_inter.pdf}
      \includegraphics[width=0.48\textwidth]{figures/ablation_final.pdf}
      \vspace{-1 ex}
      \caption{Relative accuracy of the intermediate classifier (\emph{left}) and the final classifier (\emph{right}) when introducing a single intermediate classifier at different layers in a ResNet, DenseNet and MSDNet. All experiments were performed on the CIFAR-100 dataset. Higher is better.
     }
      \vspace{-2 ex}
      \label{fig:effect-classifier}
\end{figure}


\vspace{-1ex}
\section{Multi-scale Dense Convolutional Networks}
\vspace{-1ex}
\label{sec:network}

% stolen for intro
A straightforward solution to the two problems introduced in Section~\ref{sec:setup} is to train multiple networks of increasing capacity, and sequentially evaluate them at test time (as in \cite{bolukbasi2017adaptive}). In the anytime setting the evaluation can be stopped at any point and the most recent prediction is returned. In the batch setting, the evaluation is stopped prematurely the moment a network classifies the test sample with sufficient confidence.
When the resources are so limited that the execution is terminated after the first network, this approach is optimal because the first network is trained for exactly this computational budget without compromises. However, in both settings, this scenario is rare. In the more common scenario where some test samples can require more  processing time than others the approach is far from optimal because previously learned features are never re-used across the different networks.

An alternative solution is to build a deep network with a cascade of classifiers operating on the features of internal layers: in such a network features computed for an earlier classifier can be re-used by later classifiers. However, na\"ively attaching intermediate early-exit classifiers to a state-of-the-art deep network leads to poor performance.
%We will analyze these performance-degradation problems, which will motivate several MSDNet design choices.

%\subsection{msdnet design choices}

%\subsection{The challenges of using internal features for classification}
%The MSDNet architecture is inspired by the observation that directly introducing intermediate classifiers in modern convolutional networks does not produce competitive results (in both the anytime setting and the budgeted batch classification setting) for at least two reasons.
There are two reasons why intermediate early-exit classifiers hurt the performance of deep neural networks: early classifiers lack coarse-level features and classifiers throughout interfere with the feature generation process.
In this section we investigate these effects empirically (see \figurename~\ref{fig:effect-classifier}) and, in response to our findings, propose the MSDNet architecture illustrated in Figure~\ref{fig:layout}.
%illustrates our proposed architecture which features several crucial design choices.
%which has two main components: \emph{multi-scale feature maps} and \emph{dense connectivity}. The architecture addresses the two aforementioned challenges: the multi-scale structure produces high-level features early on, whereas the dense connectivity reduces the negative effect of early classifiers on later classifiers.


\paragraph{Problem: The lack of coarse-level features.}
Traditional neural networks learn features of fine scale in early layers and coarse scale in later layers (through repeated convolution, pooling, and strided convolution). Coarse scale features in the final layers are important to classify the content of the whole image into a single class. Early layers lack coarse-level features and early-exit classifiers attached to these layers will likely yield unsatisfactory high error rates.
To illustrate this point, we attached\footnote{We select six evenly spaced locations for each of the networks to introduce the intermediate classifier. Both the ResNet and DenseNet have three resolution blocks; each block offers two tentative locations for the intermediate classifier. The loss of the intermediate and final classifiers are equally weighted.} intermediate classifiers to varying layers of a ResNet~\citep{resnet} and a DenseNet~\citep{huang2016densely} on the CIFAR-100 dataset~\citep{cifar}.
The blue and red dashed lines in the left plot of \figurename~\ref{fig:effect-classifier} show the relative accuracies of these classifiers.
 All three plots gives rise to a clear trend: the accuracy of a classifier is highly correlated with its position within the network. Particularly in the case of the ResNet (blue line), one can observe  a visible  ``staircase'' pattern,  with big improvements after the 2nd and 4th classifiers --- located right after pooling layers.

\textbf{Solution: Multi-scale feature maps.}
To address this issue, MSDNets maintain a feature representation at  \emph{multiple scales} throughout the network, and \emph{all the classifiers only use the coarse-level features}. The feature maps at a particular layer\footnote{Here, we use the term ``layer'' to refer to a column in Figure~\ref{fig:layout}.} and scale are computed by concatenating the results of one or two convolutions: 1. the result of a regular convolution applied on the same-scale features from the previous layer (horizontal connections) and, if possible, 2. the result of a strided convolution applied on the finer-scale feature map from the previous layer (diagonal connections).
The horizontal connections preserve and progress high-resolution information, which facilitates the construction of high-quality coarse features in later layers. The vertical connections produce coarse features throughout that are amenable to classification.
The dashed black line in \figurename~\ref{fig:effect-classifier} shows that MSDNets substantially increase the accuracy of early classifiers.

%noticeable benefit from simply having more layers (e.g. the improvement from the second over the first classifier), but a much more pronounced improvement arises after each pooling region (3rd over 2nd, and 5th over 4th classifier). In the case of ResNets (blue dashed line) this leads to a


%In Section~\ref{sec:results}, we will show that using this architecture for both the any time setting and the budgeted batch setting yields inferior results than the baseline of independently training multiple ResNets or DenseNets of increasing depth. From the blue curve in the left plot of \figurename~\ref{fig:effect-classifier}, we can observe that for the ResNet architecture there is a dramatic improvement (up to 10\%) when the location of the intermediate classifier moves from a high resolution block (with low level features) to a lower resolution block (with higher level features).
 %The problem can be alleviated by increasing the capacity of the classifier through stacking several convolutional and pooling layers before the fully connected layer, but these features cannot be reused by later classifiers.


% Motivated by these results, we perform an additional experiment to investigate the importance of dense connectivity and multi-scale convolutions in the context of intermediate classifiers. In particular, we train MSDNets, DenseNets and ResNets with one intermediate classifier in varying (evenly spaced) locations and observe its accuracy and the effect it has on the \emph{final} classifiers.
%For each architecture, the middle panel of \figurename~\ref{fig:ablation} shows
%the accuracy of the intermediate classifier as a function of its location (dashed lines). It also includes the accuracies of the respective final classifiers when no intermediate classifiers are introduced (dotted horizontal lines). Although all three architectures give rise to similar trends --- the intermediate classifiers improve as their relative depth increase --- there is a visible improvement obtained through the introduction of dense connectivity (from ResNet to DenseNet) and the multi-scale architecture (DenseNet to \methodnameshort{}).



%It can be observed that ResNet is affected the most, especially when the intermediate classifier is attached to high resolution feature maps (first two dots on the blue curve). Both MSDNet and DenseNet are barely affected by training with intermediate classifiers, suggesting that dense connectivity is important when one need to train internal classifiers. The right panel of \figurename~\ref{fig:ablation} show the accuracy of these internal classifiers. It is clear that MSDNet is able to produce much more accurate predictions at an early stage of the network compared to DenseNet and ResNet.




\paragraph{Problem: Early classifiers interfere with later classifiers.}
The right plot of \figurename~\ref{fig:effect-classifier}
%sheds light on to what degree the introduction of an intermediate classifier interferes with the accuracy of the final classifier: it
shows the accuracies of the \emph{final} classifier as a function of the location of a single \emph{intermediate} classifier, relative to the accuracy of a network without intermediate classifiers. The results show that the introduction of an intermediate classifier harms the final ResNet classifier (blue line), reducing its accuracy by up to $7\%$. We  postulate that this accuracy degradation in the ResNet may be caused by the intermediate classifier influencing the early features to be optimized for the short-term and not for the final layers.
%  may be caused by the intermediate classifier changing the features learned in early layers, \emph{e.g.}, by collapsing the features for some difficult samples:
This improves the accuracy of the immediate classifier but collapses information required to generate high quality features in later layers. This effect becomes more pronounced when the first classifier is attached to an earlier layer.

\textbf{Solution: Dense connectivity.}
By contrast, the DenseNet (red line) suffers much less from this effect.  Dense connectivity~\citep{huang2016densely} connects each layer with all subsequent layers and
allows later layers to \emph{bypass}  features optimized for the short-term, to maintain the high accuracy of the final classifier. If an earlier layer collapses information to generate short-term features, the lost information can be recovered through the direct connection to its preceding layer.
%If we use dense connectivity to connect every layer with every other layer
The final classifier's performance becomes (more or less) independent of the location of the intermediate classifier. As far as we know, this is the first paper that discovers that dense connectivity is an important element to early-exit classifiers in deep networks, and we make it an integral design choice in MSDNets.
%Dense connections connect each layer with all subsequent layers directly through feature concatenation , which makes \methodnameshort{}s robust against the disruptive effects of intermediate classifiers.

%Dense connections allow the model to \emph{bypass} features that are only relevant to an intermediate classifier when computing features in later layers. In addition, they significantly reduce redundant computations by encouraging feature re-use and  improve optimization by eliminating the gradient vanishing problem.

%
%Like deeply supervised networks \citep{dsn} and Inception models \citep{szegedy2015going}, our convolutional network has classifiers operating on feature maps at intermediate layers. Each of these classifiers can be used to output a prediction, which allows for retrieving preliminary predictions before a test image is propagated through the whole network. Such preliminary retrieval is essential in both the budgeted batch classification setting and the anytime prediction setting.

%\subsection{The two main components of MSDNet}


%\vspace{-2ex}
%\textbf{Challenges.}

%There are two main challenges in designing network architectures that have classifiers at various intermediate layers: 1. obtaining acceptable prediction accuracies at an early stage in the network whilst training a deep architecture, and 2. ensuring that the computation of early classifiers is not wasted when later classifiers are evaluated. The first challenge arises because classifiers that operate on low-level features (\emph{i.e.}, on features obtained before several levels of down-sampling) are generally inaccurate. The second challenge arises because feature maps in later layers generally capture different structure than features in early layers, which makes it difficult to construct classifiers that complement each other. Our convolutional networks address these two challenges via two main architectural changes: \emph{multi-scale feature maps} and \emph{dense connectivity}.
%


%\vspace{-2ex}

%Maintaining feature representations at various scales throughout the network produces the necessary low-resolution features for classification in early layers and preserves high-resolution features for the more accurate classification in later layers.
% higher quality features (that rely on the earlier high-resolution feature maps) later in the network.


%\vspace{-2ex}

% around these intermediate layers prevent them from becoming bottlenecks and remove the negative side-effects that earlier classifiers otherwise have on later classifiers.

% the use of dense connections is instrumental in addressing the second challenge identified above: dense connections differ from traditional network architectures in that they add additional features at each layer whilst maintaining all features that were computed prior. Moreover, learning this intermediate classifier barely hurt the performance of the regular classifier at the end of the network.

%This facilitates a very natural way of training classifiers at different layers that complement each other without wasting computation: we share the weights between the linear classifiers at different layers. As a result, to perform predictions using one of the classifiers, we only need to compute the inner product between the ``new'' features and the associated classifier weights and can add the result to the output of the previous classifier in the network. This allows us to progressively update the predictions of the network as we propagate the input through the network, which makes our networks suitable for anytime predictions.

%\vspace{-2ex}
%\textbf{Parameter efficiency.} Perhaps somewhat counterintuitively, our architectural changes improve the parameter efficiency significantly. In particular, a version of our network with less than 1 million parameters is able get lower than $7.0\%$ test error on CIFAR-10 dataset, which suggests our architecture is on par with or better than existing architectures in terms of the accuracy-model size trade-off (for instance, \citep{saxena2016convolutional} reported a $7.43\%$ test error on the same dataset using a model with $>$20 million parameters). We present the details of our \methodnameshort{} below.

%The proposed cost sensitive CNN is a network with multiple outputs, which are (usually uniformly) distributed along the depth of network. Each of the outputs has its own classification layer, and can independently give predictions for any given input. Therefore, this architecture allows for retrieving results at an early stage before propagating a test image through all the convolutional layers. Note that similar architectures have been adopted in many existing CNNs, e.g., Deeply Supervised Net (DSN) \citep{dsn} and the Inception model \citep{szegedy2015going}. However, these networks are not oriented for test time cost sensitive learning, and the accuracy of early classification is not addressed.

%The main challenge in realizing cost sensitive learning with CNNs is that it has the hierarchical structure to learn features from low level to high level. Building a classification layer on top of low level features before down-sampling usually yields poor test performance. Therefore, simply attach multiple classification layers to a typical CNN can not ensure accurate predictions for early exits.

%To solve this problem, we introduce a novel CNN architecture with many down-sampling layers along the depth of network, but with minimum redundancy to achieve highly efficient inference at test time. The proposed \methodnameshort{} as shown in Fig.~\ref{fig:layout} is inspired by the Convolutional Neural Fabrics \citep{saxena2016convolutional}, but we made substantial changes to make it suitable for test time cost sensitive learning. The most important change is that we introduce \emph{dense connections} \citep{huang2016densely} to allow each layer \footnote{Here we use the term 'layer' to refer to a column shown on the graph.} receiving inputs directly from all its previous layers. The dense connectivity brings at least two notable advantages: 1) it significantly reduces redundant computations by encouraging feature reusing, as shown in \citep{huang2016densely}; 2) it makes the optimization easier with the long range connections. Without dense connections, the performance of the network starts to deteriorate when the depth exceed 20 layers. More details about the proposed \methodnameshort{} are given below. It is noteworthy that our base network (with one single classification layer at the end) with less than 1M parameters is able get lower than 7.0\% test error on CIFAR-10 dataset, while \citep{saxena2016convolutional} reported a 7.43\% test error on the same dataset using a CNF with $>$20M parameters.

%Second, there is a trade-off between the accuracy of classification layers at shallower layers and those at deeper layers. If we put too much weight on achieving high performance at an early stage, then the convolutional layers near the input of the network will try to learn too aggressive features, making the later layers difficult to adapt.


\renewcommand{\arraystretch}{1.1}
\begin{figure}[!t]
%\vspace{1 ex}
\centerline{
\includegraphics[width=1\textwidth]{figures/figure2.pdf}}
\caption{The output $\bx_{\ell}^{s}$ of layer $\ell$ at the $s^\text{th}$ scale in a \methodnameshort{}. Herein, $[ \dots ]$ denotes the concatenation operator, $h_{\ell}^s(\cdot)$ a regular convolution transformation, and $\tilde{h}_{\ell}^s(\cdot)$ a strided convolutional. Note that the outputs of $h_{\ell}^s$ and $\tilde{h}_{\ell}^s$ have the same feature map size; their outputs are concatenated along the channel dimension. }

% \resizebox{0.6\textwidth}{!}{%
% \begin{tabular}{lcc}
%     \toprule
%     & $s=1$ & $s>1$ \\
%                     \midrule
%   $\ell = 1$       & $h_0(\bx_{0}^{1})$ & $\tilde{h}_0(\bx_{1}^{(s-1)})$  \\
%   $\ell > 1$ & $h_{\ell}(\left[\bx_{1}^{s},\ldots, \bx_{\ell-1}^{s}\right]\right)$
%                     & $\left[ \begin{array}{l}
%             h_{\ell}\left(\left[\bx_{1}^{s},\ldots, \bx_{\ell-1}^{s}\right]\right), \\
%             \tilde{h}_{\ell}\left(\left[\bx_{1}^{(s-1)},\ldots, \bx_{\ell-1}^{(s-1)}\right]\right)\\
%             \end{array}
%         \right]$ \\
%             \bottomrule
% \end{tabular}
% }
\label{tab:layers}
\vspace{-3 ex}
\end{figure}


%\begin{wraptable}{r}{5.5cm}
%\begin{tabular}{ccc}\\\toprule
%\end{tabular}
%\end{wraptable}

\subsection{the msdnet architecture}
\label{subsec:arch}
%We present the details of \methodnameshort{} below.

The MSDNet architecture is illustrated in \autoref{fig:layout}. We present its main components below. Additional details on the architecture are presented in Appendix~\ref{sec:archdetails}.

%\vspace{-2ex}
\textbf{First layer.}
The first layer ($\ell \! = \! 1$) is unique as it includes vertical connections in Figure~\ref{fig:layout}. Its main purpose is to ``seed'' representations on all $S$ scales. One could view its vertical layout as  a miniature ``S-layers'' convolutional network (S=3 in Figure~\ref{fig:layout}).
Let us denote the output feature maps at layer $\ell$ and scale $s$ as $\bx_\ell^{s}$ and the original input image as $\bx_0^1$.
%The first scale receives the input image $\bx_0^1$ and passes on its output to the  feature maps at the input scale $s \! = \! 1$ and at coarser scales $s \! > \! 1$.
Feature maps at coarser scales are obtained via down-sampling. The output $\bx_{1}^{s}$ of the first layer  is formally given in the top row of Figure~\ref{tab:layers}.

%\vspace{-1ex}
%\begin{equation}
%\bx_{1}^{s} = \left\{\begin{array}{ll}
%              h_0(\bx_{0}^{1}) & \mbox{if } s=1, \\
%              \tilde{h}_0(\bx_{1}^{(s-1)}) & \mbox{if $s>1$}.
%             \end{array} \right.
%\label{eqn:output1}\nonumber
%%\vspace{-1ex}
%\end{equation}
%\begin{equation}
%\bx_{1}^{s} =  h_0(\bx_{0}^{1}), \quad \emph{if} \quad s=1; \qquad or \quad
%             gi \bx_{1}^{s} = \tilde{h}_0(\bx_{1}^{(s-1)}), \quad \emph{if} \quad s>1.
%\label{eqn:output1}\nonumber
%%\vspace{-1ex}
%\end{equation}

%Herein, $h_0(\cdot)$ and $\tilde h_0(\cdot)$ denote a regular convolutional transformation and a strided convolutional transformation, respectively. The output of the first layer is a collection giof feature maps $\left\{\bx_1^{1}, \dots, \bx_1^{S}\right\}$, one for each scale.

%\vspace{-2ex}
\textbf{Subsequent layers.}
%As pointed out in~\citep{huang2016densely}, connecting layer $\ell$ with layer $\ell+1$ and $\ell+2$ is identical to concatenating
Following~\citet{huang2016densely},
the output feature maps $\bx_\ell^{s}$ produced at subsequent layers, $\ell\!>\!1$, and scales, $s$, are a concatenation of transformed feature maps from all previous feature maps of scale $s$ and $s-1$ (if $s>1$).
Formally, the $\ell$-th layer of our network outputs a set of features at $S$ scales $\left\{\bx_\ell^{1},\ldots, \bx_\ell^{S}\right\}$, given in the last row of Figure~\ref{tab:layers}.

%\vspace{-1ex}
%\begin{equation}
%\bx_{\ell}^{s} = \left\{\begin{array}{ll}
%         \begin{array}{l}
%               h_{\ell}\left(\left[\bx_{1}^{s},\ldots, \bx_{\ell-1}^{s}\right]\right)\\
%        \end{array}
%         & \mbox{if } s=1, \\
%        \ \\ \vspace{-1ex}
%        \left[ \begin{array}{l}
%            h_{\ell}\left(\left[\bx_{1}^{s},\ldots, \bx_{\ell-1}^{s}\right]\right), \\
%            \tilde{h}_{\ell}\left(\left[\bx_{1}^{(s-1)},\ldots, \bx_{\ell-1}^{(s-1)}\right]\right)\\
%            \end{array}
%        \right] & \mbox{$s>1$}.
%             \end{array} \right.
%\label{eqn:output}\nonumber
%\end{equation}


%Note that the up-sampling paths are \emph{not} used for classification tasks in our experiments, as generally they are mostly useful for segmentation tasks. In our experiment, each input path produces an equal number of output channels for a given layer and scale.

%\vspace{-2ex}
\textbf{Classifiers.} The classifiers in \methodnameshorts{} also follow the dense connectivity pattern within the coarsest scale, $S$, i.e., the classifier at layer $\ell$ uses all the features $\left[\bx_1^{S},\ldots,\bx_\ell^{S}\right]$. Each classifier consists of two convolutional layers, followed by one average pooling layer and one linear layer. In practice, we only attach classifiers to some of the intermediate layers, and we let $f_k(\cdot)$ denote the $k^\text{th}$ classifier.
During testing in the \emph{anytime} setting we propagate the input through the network until the budget is exhausted and output the most recent prediction.
%
In the \emph{batch budget} setting at test time, an example traverses the network and exits after classifier $f_k$ if its prediction confidence (we use the maximum value of the softmax probability as a confidence measure) exceeds a pre-determined threshold $\theta_k$. Before training, we compute the computational cost, $C_k$, required to process the network up to the $k^\text{th}$ classifier. We denote by $0 \!< \! q\leq 1$ a fixed \emph{exit probability} that a sample that \emph{reaches} a classifier will obtain a classification with sufficient confidence to exit. We assume that $q$ is constant across all layers, which allows us to compute the probability that a sample exits at classifier $k$ as: $q_k=z(1-q)^{k-1}q$,
%\vspace{-1ex}
%\begin{equation}
%  q_k=z(1-q)^{k-1}q,\label{eq:ql}
%\end{equation}
where $z$ is a normalizing constant that ensures that $\sum_k p(q_k) = 1$. At test time, we need to ensure that the overall cost of classifying all samples in $\mathcal{D}_{test}$ does not exceed our budget $B$ (in expectation). This gives rise to the constraint $|\mathcal{D}_{test}| \sum\nolimits_{k} q_k C_k\leq B$. We can solve this constraint for $q$ and determine the thresholds $\theta_k$ on a validation set in such a way that approximately $|\mathcal{D}_{test}| q_{k}$ validation samples exit at the $k^\text{th}$ classifier.
%In preliminary experiments, we also experimented with entropy-based confidence measures and class-specific thresholds, but we did not find these approaches to work better.

%This provides a natural way to determine the required depth of the network: as $q_k$ is exponentially decreasing, one can set the final layer to be the first layer with $q_k \! < \! \epsilon$, for some small $\epsilon \! > \! 0$.
% LAURENS: I uncommented the above sentence because I don't think it is entirely true: it also depends on how many classifiers you attach to the network?

%\vspace{-1ex}
%\begin{equation}
% |\mathcal{D}_{test}| \sum\nolimits_{k} q_k C_k\leq B.\label{eq:budget}
%%\vspace{-1ex}
%\end{equation}


%\vspace{-2ex}
\textbf{Loss functions.}
During training we use cross entropy loss functions $L(f_k)$ for all classifiers and minimize a weighted cumulative loss: $\frac{1}{\mathcal{|D|}}\sum\nolimits_{(\bx,y)\in\mathcal{D}} \sum\nolimits_{k}w_k L(f_k)$. Herein, $\mathcal{D}$ denotes the training set and $w_k\!\geq\! 0$ the weight of the $k$-th classifier. If the budget distribution $P(B)$ is known, we can use the weights $w_k$ to incorporate our prior knowledge about the budget $B$ in the learning.
%In the batch computational budget setting, the budget $B$ is known before test time, which allows for the design of proper weights to adapt for the given budget. In the anytime setting, the budget $B$ is sampled from some distribution $P(\bx, B)$. When the marginal distribution $P(B)$ is known, we can adapt the weights $w_k$ accordingly.
Empirically, we find that using the same weight for all loss functions (\emph{i.e.}, setting $\forall k\!: w_k \! = \! 1$) works well in practice.

%We can compute the exit probabiligities $q_\ell$ as described in the  previous paragraph and assign the weights $w_\ell=q_\ell$ to be the probability that a test sample will exit at layer $\ell$. In practice this provides an elegant way to determine the required depth of the network: As $w_\ell$ is exponentially decreasing, one can set the final layer $L$ to be the first layer with $w_L<\epsilon$, for some small $\epsilon>0$.

% which down-sample the features to $1\times 1$ scale, followed by a fully connected linear layer.


%We use linear classifiers at different layers in the network. These classifiers perform an average pooling of the feature maps at coarsest scale ($S$) of layer $\ell$, and compute the inner product between a weight matrix and the resulting pooled features. We apply a softmax on the resulting scores to obtain a distribution over classes.
%
%Recall that the feature maps are produced by concatenations: that is, feature maps take the form $\left[\bx_1^{S},\ldots,\bx_\ell^{S}\right]$. As a result, we can share the weights that are applied to a particular feature map between classifiers. In other words, the weights $\mathbf{w}_1$ applied to the pooled features $\bx_1^{S}$ are the same for all classifiers, the weights $\mathbf{w}_2$ applied to $\bx_2^{S}$ are the same for all classifiers, etc. The classifier weight sharing makes updating the network's predictions during forward propagation of the inputs very efficient: to compute the output of a classifier, we only need to add the inner product of its weights with ``new'' (pooled) feature maps to the output of the previous classifier.

%We find that using features from more scales does not improve the performance but significantly increases the computation cost. This also verifies that low level features are indeed less discriminative for classification.

%\textbf{Loss function.} The goal of learning is to minimize the expected loss of Equation~(\ref{eqn:objective}). We use a logistic loss function $L(\cdot)$ and estimate the expectation over $P(\mathbf{x})$ by an empirical average over the training data. Similarly, we estimate the expectation over $P(B)$ by an average over the ``realizable'' budgets $B$: that is, we only consider budgets $B$ corresponding to classifiers in the network in the expectation. We perform experiments with four different  budget distributions $P(B)$, namely, an exponential distribution, a uniform distribution and a normal distribution.





%\vspace{-2ex}
\textbf{Network reduction and lazy evaluation.} There are two straightforward ways to further reduce the computational requirements of \methodnameshort{}s. First, it is inefficient to maintain all the finer scales until the last layer of the network. One simple strategy to reduce the size of the network is by splitting it into $S$ blocks along the depth dimension, and only keeping the coarsest $(S-i+1)$ scales in the $i^\text{th}$ block (a schematic layout of this structure is shown in \autoref{fig:reduction}). This reduces computational cost for both training and testing. Every time a scale is removed from the network, we add a transition layer between the two blocks that merges the concatenated features using a $1 \!\times\! 1$ convolution and cuts the number of channels in half before feeding the fine-scale features into the coarser scale via a strided convolution (this is similar to the DenseNet-BC architecture of \citet{huang2016densely}). Second, since a classifier at layer $\ell$ only uses features from the coarsest scale, the finer feature maps in layer $\ell$ (and some of the finer feature maps in the previous $S \!-\! 2$ layers) do not influence the prediction of that classifier. Therefore, we group the computation in ``diagonal blocks'' such that we only propagate the example along paths that are required for the evaluation of the next classifier. This minimizes unnecessary computations when we need to stop because the computational budget is exhausted. We call this strategy \emph{lazy evaluation}.
%Therefore, we compute the feature set $\{\bx_{\ell+1}^{1},\ldots,\bx_{\ell+S}^{S}\}$ in parallel, avoiding unnecessary computations when we need to stop at the $(\ell+S)^{th}$ scale to retrieve the prediction.

%% moved to supplementary
%%\vspace{-2ex}
%\textbf{Implementation details.}
%We use \methodnameshort{} with three scales on the CIFAR datasets.
%The convolutional layer functions in the first layer, $h_{1}$, denote a sequence of $3 \! \times \! 3$ convolutions (Conv), batch normalization (BN;~\citep{batch-norm}), and rectified linear unit (ReLU) activation. In the computation of $\tilde h_{1}$, down-sampling is performed by performing convolutions using strides that are powers of two. For subsequent feature layers, the transformations $h_{\ell}$ and $\tilde h_{\ell}$ are defined following the design in DenseNets \citep{huang2016densely}: Conv($1\times 1$)-BN-ReLU-Conv($3\times 3$)-BN-ReLU. We set the number of output channels of the three scales to 6, 12, and 24, respectively. Each classifier has two down-sampling convolutional layers with 128 dimensional $3 \! \times \! 3$ filters, followed by a $2 \! \times \! 2$ average pooling layer and a linear layer.
%The \methodnameshort{} used for ImageNet has four scales, respectively producing 16, 32, 64, and 64 feature maps at each layer. The original images are first transformed by a 7$\times$7 convolution and a 3$\times$3 max pooling (both with stride 2), before entering the first layer of \methodnameshort{}s. The classifiers have the same structure as those used for the CIFAR datasets, except that the number of output channels of each convolutional layer is set to be equal to the number of its input channels.

%[To do] For segmentation tasks...


==> Cost_Sensitive_CNN - arXiv-20180607/related_work.tex <==
%!TEX root=main.tex

\vspace{-1ex}
\section{Related Work}
\vspace{-1ex}
We briefly review related prior work on computation-efficient networks, memory-efficient networks, and resource-sensitive machine learning, from which our network architecture draws inspiration.

%\vspace{-2ex}
\textbf{Computation-efficient networks.}
Most prior work on (convolutional) networks that are computationally efficient at test time focuses on reducing model size after training. In particular, many studies propose to prune weights~\citep{lecun1989optimal,hassibi1993optimal,li2016pruning} or quantize weights~\citep{hubara2016binarized,rastegari2016xnor} during or after training.
These approaches are generally effective because deep networks often have a substantial number of redundant weights that can be pruned or quantized without sacrificing (and sometimes even improving) performance. Prior work also studies approaches that directly learn \emph{compact} models with less parameter redundancy. For example, the knowledge-distillation method \citep{bucilu2006model,hinton2015distilling} trains small student networks to reproduce the output of a much larger teacher network or ensemble.
Our work differs from those approaches in that we train a single model that trades off computation for accuracy at test time without any re-training or finetuning. Indeed, weight pruning and knowledge distillation can be used in combination with our approach, and may lead to further improvements.

%The DenseNet architecture \citep{huang2016densely} by design encourages heavy feature reusing in the network, leading to highly compact models.

%%\vspace{-2ex}
%\textbf{Memory-efficient networks.}
%A large body of recent prior work explores memory-efficient (convolutional) network architectures. Most of these studies perform some type of quantization of the network's weights \citep{gong2014compressing} or use hashing~\citep{chen2015compressing,chen2016compressing}
%% LAURENS: There are many other papers doing this. Have a look at the list at https://www.reddit.com/r/MachineLearning/comments/3oiefh/quantization_then_reduces_the_number_of_bits_that/cvxjd8z/
%with some even going as far as to train networks with binary weights \citep{hubara2016binarized,rastegari2016xnor}. \citet{rastegari2016xnor} recently showed that a binary-weight version of AlexNet \citep{alexnet} can match the performance of its $32$-bits floating point counterpart on the ImageNet dataset. Whereas memory efficiency is essential for deploying deep networks on mobile platforms, quantization generally often leads to a decrease in computational efficiency because weights quantization requires additional look-up operations before the network can be evaluated. In this study, we do not focus on memory efficiency although we believe that existing weight quantization approaches can be used successfully with our network architecture in case memory efficiency is important.

%\vspace{-2ex}
\textbf{Resource-efficient machine learning.}
Various prior studies explore computationally efficient variants of traditional machine-learning models \citep{viola2001robust,grubb2012speedboost,karayev2014anytime,trapeznikov2013supervised,ICML2012Xu_592,xu2013cost,icml2015_nan15,wang2015acyclic}. Most of these studies focus on how to incorporate the computational requirements of computing particular features in the training of machine-learning models such as (gradient-boosted) decision trees. Whilst our study is certainly inspired by these results, the architecture we explore differs substantially: most prior work exploits characteristics of machine-learning models (such as decision trees) that do not apply to deep networks. Our work is possibly most closely related to recent work on FractalNets \citep{fractalnet}, which can perform anytime prediction by progressively evaluating subnetworks of the full network. FractalNets differ from our work in that they are not explicitly optimized for computation efficiency and consequently our experiments show that \methodnameshorts{} substantially outperform FractalNets. Our dynamic evaluation strategy for reducing batch computational cost is closely related to the the \emph{adaptive computation time} approach \citep{graves2016adaptive,figurnov2016spatially}, and the recently proposed method of adaptively evaluating neural networks \citep{bolukbasi2017adaptive}.
\filler{Different from these works, our method adopts a specially designed network with multiple classifiers, which are jointly optimized during training and can directly output confidence scores to control the evaluation process for each test example.}
%
The \emph{adaptive computation time} method \citep{graves2016adaptive} and its extension \citep{figurnov2016spatially} also perform adaptive evaluation on test examples to save batch computational cost, but focus on skipping units rather than layers. In \citep{odena2017changing}, a ``composer''model is trained to construct the evaluation network from a set of sub-modules for each test example. By contrast, our work uses a single CNN with multiple intermediate classifiers that is trained end-to-end. The Feedback Networks \citep{2016arXiv161209508Z} enable early predictions by making predictions in a recurrent fashion, which heavily shares parameters among classifiers, but is less efficient in sharing computation.

%Our method differs from these works in that we have a specially designed network with multiple classifiers, which can be easily trained in a end-to-end manner.

%\vspace{-2ex}
\textbf{Related network architectures.} Our network architecture borrows elements from neural fabrics \citep{saxena2016convolutional} and others \citep{zhou2015interlinked,jacobsen2017multiscale,ke2016neural} to rapidly construct a low-resolution feature map that is amenable to classification, whilst also maintaining feature maps of higher resolution that are essential for obtaining high classification accuracy.  Our design differs from the neural fabrics~\citep{saxena2016convolutional} substantially in that \methodnameshort{}s have a reduced number of scales and no sparse channel connectivity or up-sampling paths. \methodnameshort{}s are  at least one order of magnitude more efficient and typically more accurate
 --- for example, an \methodnameshort{} with less than 1 million parameters obtains a test error below $7.0\%$ on CIFAR-10~\citep{cifar}, whereas \citet{saxena2016convolutional} report $7.43\%$  with  over $20$ million parameters.
We use the same feature-concatenation approach as DenseNets \citep{huang2016densely}, which allows us to bypass features optimized for early classifiers in later layers of the network.
%A similar way of reusing features is used in progressive networks \citep{rusu2016progressive}.
Our architecture is related to deeply supervised networks \citep{dsn} in that it incorporates classifiers at multiple layers throughout the network. In contrast to all these prior architectures, our network is specifically designed to operate in resource-aware settings.



%\subsection{Neural Fabrics}
%
%\begin{figure}[t]
%%\vspace{-2 ex}
%      \centering
%      \includegraphics[width=0.5\textwidth]{figures/cnf.pdf}
%      \caption{Convolutional neural fabrics. }
%      \label{fig:cnf}
%%      \vspace{-2 ex}
%\end{figure}
%
%\subsection{DenseNet}


==> Cost_Sensitive_CNN - arXiv-20180607/results.tex <==
%!TEX root=main.tex
\vspace{-1ex}
\section{Experiments}
\label{sec:results}
\vspace{-1ex}

We evaluate the effectiveness of our approach on three image classification datasets, i.e., the CIFAR-10, CIFAR-100~\citep{cifar} and ILSVRC 2012 (ImageNet; \citet{deng2009imagenet}) datasets. Code to reproduce all results is available at \url{https://anonymous-url}.
Details on architectural configurations of MSDNets are described in Appendix \ref{sec:archdetails}.

\paragraph{Datasets.}
The two CIFAR datasets contain $50,000$ training and $10,000$ test images of $32 \! \times \! 32$ pixels; we hold out $5,000$ training images as a validation set. The datasets comprise $10$ and $100$ classes, respectively. We follow \cite{resnet} and apply standard data-augmentation techniques to the training images: images are zero-padded with 4 pixels on each side, and then randomly cropped to produce 32$\times$32 images. Images are flipped horizontally with probability $0.5$, and normalized by subtracting channel means and dividing by channel standard deviations. The ImageNet dataset comprises $1,000$ classes, with a total of 1.2 million training images and 50,000 validation images. We hold out 50,000 images from the training set to estimate the confidence threshold for classifiers in \methodnameshort{}. We adopt the data augmentation scheme of \cite{resnet} at training time; at test time, we classify a $224 \! \times \! 224$ center crop of images that were resized to $256 \! \times \! 256$ pixels.

\paragraph{Training Details.}
We train all models using the framework of \cite{blogresnet}. On the two CIFAR datasets, all models (including all baselines) are trained using stochastic gradient descent (SGD) with mini-batch size 64. We use Nesterov momentum with a momentum weight of 0.9 without dampening, and a weight decay of 10$^{-4}$. All models are trained for 300 epochs, with an initial learning rate of 0.1, which is divided by a factor 10 after $150$ and $225$ epochs. We apply the same optimization scheme to the ImageNet dataset, except that we increase the mini-batch size to 256, and all the models are trained for 90 epochs with learning rate drops after $30$ and $60$ epochs.





%\input{archdetails}
\input{anytimeresults}
\input{batchresults}





\subsection{More Computationally Efficient DenseNets}
Here, we discuss an interesting finding during our exploration of the MSDNet architecture. We found that following the DenseNet structure to design our network, \emph{i.e.}, by keeping the number of output channels (or \emph{growth rate}) the same at all scales, did not lead to optimal results in terms of the accuracy-speed trade-off. The main reason for this is that compared to network architectures like ResNets, the DenseNet structure tends to apply more filters on the high-resolution feature maps in the network. This helps to reduce the number of parameters in the model, but at the same time, it greatly increases the computational cost. We tried to modify DenseNets by doubling the growth rate after each transition layer, so that more filters are applied to low-resolution feature maps. It turns out that the resulting network, which we denote as DenseNet*, significantly outperform the original DenseNet in terms of computational efficiency.

We experimented with DenseNet* in our two settings with test time budget constraints. The left panel of
\figurename~\ref{fig:densenet-opt} shows the anytime prediction performance of an ensemble of DenseNets* of varying depths. It outperforms the ensemble of original DenseNets of varying depth by a large margin, but is still slightly worse than MSDNets. In the budgeted batch budget setting, DenseNet* also leads to significantly higher accuracy over its counterpart under all budgets, but is still substantially outperformed by MSDNets.

 \begin{figure*}[t]
      \centering
%\vspace{-2 ex}
      \includegraphics[width=0.48\textwidth]{figures/anytime-cifar100-append.pdf}
      \includegraphics[width=0.48\textwidth]{figures/early-exit-cifar100-append.pdf}\\
      \caption{Test accuracy of DenseNet* on CIFAR-100 under the anytime learning setting (\emph{left}) and the budgeted batch setting (\emph{right}).}
  %     \vspace{-2 ex}
     \label{fig:densenet-opt}
\end{figure*}

